A Hybrid Discrete Exterior Calculus Discretization and Fourier Transform of the Incompressible Navier-Stokes Equations in 3D

The simulation of fluid flow problems, specifically incompressible flows governed by the Navier-Stokes equations (NSE), holds fundamental significance in a range of scientific and engineering applications. Traditional numerical methods employed for solving these equations on three-dimensional (3D) meshes are commonly known for their moderate conservation properties, high computational intensity and substantial resource demands. Relying on its ability to capture the intrinsic geometric and topological properties of simplicial meshes, discrete exterior calculus (DEC) provides a discrete analog to differential forms and enables the discretization of partial differential equations (PDEs) on meshes.We present a hybrid discretization approach for the 3D incompressible Navier-Stokes equations based on DEC and Fourier transform (FT). An existing conservative primitive variable DEC discretization of incompressible Navier-Stokes equations over surface simplicial meshes developed by Jagad et al. [1] is considered in the planar dimension while the Fourier expansion is applied in the third dimension. The test cases of three-dimensional lid-driven cavity and viscous Taylor-Green three-dimensional vortex (TGV) flows show that the simulation results using this hybrid approach are comparable to literature.

==> Abstract.tex <==

% Abstract File
% Do not remove centering environment below
\begin{center}

\end{center}

\begin{center}
{{\bf\fontsize{14pt}{14.5pt}\selectfont \uppercase{ABSTRACT}}}
\end{center}

\doublespacing
\addcontentsline{toc}{chapter}{Abstract}



\begin{center}
	\begin{doublespace}
{\fontsize{14pt}{14.5pt}\selectfont {A Hybrid Discrete Exterior Calculus Discretization and Fourier Transform of the Incompressible Navier-Stokes Equations in 3D}}\\
		{\fontsize{14pt}{14.5pt}\selectfont {Abdullah Hassan Ibrahim Abukhwejah}}\\
%		{\fontsize{12pt}{12.5pt}\selectfont {Ph.D. Year}}\\
	\end{doublespace}
\end{center}
The simulation of fluid flow problems, specifically incompressible flows governed by the Navier-Stokes equations (NSE), holds fundamental significance in a range of scientific and engineering applications. Traditional numerical methods employed for solving these equations on $three{\text -}dimensional$ (3D) meshes are commonly known for their moderate conservation properties, high computational intensity and substantial resource demands. Relying on its ability to capture the intrinsic geometric and topological properties of simplicial meshes, discrete exterior calculus (DEC) provides a discrete analog to differential forms and enables the discretization of partial differential equations (PDEs) on meshes. We present a hybrid discretization approach for the 3D incompressible Navier-Stokes equations based on DEC and Fourier transform (FT). An existing conservative primitive variable DEC discretization of incompressible Navier–Stokes equations over surface simplicial meshes developed by Jagad et al. \cite{jagad2021primitive} is considered in the planar dimension while the Fourier expansion is applied in the third dimension. The test cases of three-dimensional lid-driven cavity and viscous Taylor-Green three-dimensional vortex (TGV) flows show that the simulation results using this hybrid approach are comparable to literature.

==> Acknowledgment.tex <==

% Acknowledgments File


\begin{center}

\end{center}
\begin{center}

{\bf\fontsize{14pt}{14.5pt}\selectfont \uppercase{Acknowledgements}}\\\vspace{1cm}
\end{center}

\addcontentsline{toc}{chapter}{Acknowledgements} % (Optional)

``So high [above all] is Allah, the Sovereign, the Truth. And, [O Muhammad], do not hasten with [recitation of] the Qur'an before its revelation is completed to you, and say, ``My Lord, increase me in knowledge'''' \cite{increaseme}.
\\
``And they ask you, [O Muhammad], about the soul. Say, ``The soul is of the affair of my Lord. And mankind have not been given of knowledge except a little'''' \cite{Andtheyaskyou}.
\\
Abu Hurairah (May Allah be pleased with him) narrated: The Messenger of
Allah (peace be upon him) said ``When a son of Adam (i.e. any human being) dies his deeds are discontinued, with three exceptions: Sadaqah, whose benefit is continuous; or knowledge from which benefit continues to be reaped, or a righteous child who supplicates for him''\cite{AbuHurairah} and in another narration ``Whoever takes a path upon which to obtain knowledge, Allah makes the path to Paradise easy for him'' \cite{AbuHurairah2}.

``KAUST shall be a beacon for peace, hope and reconciliation, and shall serve the
people of the Kingdom and the world'' King Abdullah bin Abdulaziz Al Saud

I express my heartfelt gratitude to Allah, the Supreme and All-Powerful Being, for the unending stream of blessings He has bestowed upon me. Additionally, I extend my deep appreciation to the individual whom I hold in the highest esteem—Prophet Mohammad. His teachings have left a profound impact on me, and I embrace and adhere to the principles he imparted.

A substantial portion of my accomplishments can be attributed to the unwavering support and guidance provided by my parents, both my father and mother. Their encouragement to pursue knowledge and their consistent message to never surrender have been instrumental in shaping my achievements.

Furthermore, I must acknowledge the pivotal role played by my beloved wife and son throughout my journey toward obtaining my PhD. They have held a central position in this significant undertaking, offering support, inspiration, and motivation that have been indispensable to my success.

King Abdullah merits a significant portion of my supplications, not solely due to his role in elevating KAUST to a globally renowned university, but also for revitalizing the Islamic enthusiasm for the pursuit of knowledge. I express my gratitude to Professor Ravi Samtaney and Professor Peter Schmid for welcoming me as their student. Their freshness of thought, amazing knowledge, vision, flexibility, and patience have been crucial to this work. Besides providing me valuable advice, and guidance throughout my Ph.D. journey, they have been a constant source of motivation. I also extend my appreciation to the members of the committee members, namely Professor Hussein Hoteit, Professor Hong Im, and Professor Anil Hirani for the their great support, advise and being great teachers.

Many thanks go to all my colleagues in the Fluid Plasma Simulation lab, as well, specifically Dr. Pankaj Jagad for his direct contributions in this work.
\\
I am also grateful to King AbdulAziz City for Science and Technology (KACST) and KAUST for providing me with the financial support that made this research possible.


==> Figs/TGV/ux_vs_y_TGV.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(682,797){\makebox(0,0)[r]{\strut{}$-3$}}%
      \put(682,1452){\makebox(0,0)[r]{\strut{}$-2$}}%
      \put(682,2107){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(682,2762){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(682,3416){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(682,4071){\makebox(0,0)[r]{\strut{}$2$}}%
      \put(682,4726){\makebox(0,0)[r]{\strut{}$3$}}%
      \put(814,484){\makebox(0,0){\strut{}$-1$}}%
      \put(2311,484){\makebox(0,0){\strut{}$-0.5$}}%
      \put(3809,484){\makebox(0,0){\strut{}$0$}}%
      \put(5306,484){\makebox(0,0){\strut{}$0.5$}}%
      \put(6803,484){\makebox(0,0){\strut{}$1$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(198,2761){\rotatebox{-270}{\makebox(0,0){\strut{}$y$}}}%
      \put(3808,154){\makebox(0,0){\strut{}$u_x$}}%
      \csname LTb\endcsname%%
      \put(1729,4656){\makebox(0,0)[l]{\strut{} }}%
      \csname LTb\endcsname%%
      \put(1729,4456){\makebox(0,0)[l]{\strut{}Analytical}}%
      \csname LTb\endcsname%%
      \put(1729,4256){\makebox(0,0)[l]{\strut{}Computed}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{Figs/TGV/ux_vs_y_TGV.pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figs/TGV/uy_vs_x_TGV.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(946,704){\makebox(0,0)[r]{\strut{}$-1$}}%
      \put(946,1733){\makebox(0,0)[r]{\strut{}$-0.5$}}%
      \put(946,2762){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(946,3790){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \put(946,4819){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(1207,484){\makebox(0,0){\strut{}$-3$}}%
      \put(2118,484){\makebox(0,0){\strut{}$-2$}}%
      \put(3029,484){\makebox(0,0){\strut{}$-1$}}%
      \put(3941,484){\makebox(0,0){\strut{}$0$}}%
      \put(4852,484){\makebox(0,0){\strut{}$1$}}%
      \put(5763,484){\makebox(0,0){\strut{}$2$}}%
      \put(6674,484){\makebox(0,0){\strut{}$3$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(198,2761){\rotatebox{-270}{\makebox(0,0){\strut{}$u_y$}}}%
      \put(3940,154){\makebox(0,0){\strut{}$x$}}%
      \csname LTb\endcsname%%
      \put(1993,4656){\makebox(0,0)[l]{\strut{} }}%
      \csname LTb\endcsname%%
      \put(1993,4456){\makebox(0,0)[l]{\strut{}Analytical}}%
      \csname LTb\endcsname%%
      \put(1993,4256){\makebox(0,0)[l]{\strut{}Computed}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{Figs/TGV/uy_vs_x_TGV.pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figs/cavity/u_vs_y_2Dghia.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7500.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1078,704){\makebox(0,0)[r]{\strut{}$-0.5$}}%
      \put(1078,1733){\makebox(0,0)[r]{\strut{}$-0.25$}}%
      \put(1078,2762){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(1078,3790){\makebox(0,0)[r]{\strut{}$0.25$}}%
      \put(1078,4819){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \put(1210,484){\makebox(0,0){\strut{}$-0.6$}}%
      \put(1909,484){\makebox(0,0){\strut{}$-0.4$}}%
      \put(2608,484){\makebox(0,0){\strut{}$-0.2$}}%
      \put(3307,484){\makebox(0,0){\strut{}$0$}}%
      \put(4007,484){\makebox(0,0){\strut{}$0.2$}}%
      \put(4706,484){\makebox(0,0){\strut{}$0.4$}}%
      \put(5405,484){\makebox(0,0){\strut{}$0.6$}}%
      \put(6104,484){\makebox(0,0){\strut{}$0.8$}}%
      \put(6803,484){\makebox(0,0){\strut{}$1$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(198,2761){\rotatebox{-270}{\makebox(0,0){\strut{}$y/L$}}}%
      \put(4006,154){\makebox(0,0){\strut{}$u_x$}}%
      \csname LTb\endcsname%%
      \put(5111,3661){\makebox(0,0)[l]{\strut{} Ghia et al. \cite{ghia1982high}}}%
      \csname LTb\endcsname%%
      \put(5111,3461){\makebox(0,0)[l]{\strut{}$Re = 100$}}%
      \csname LTb\endcsname%%
      \put(5111,3261){\makebox(0,0)[l]{\strut{}$Re = 400$}}%
      \csname LTb\endcsname%%
      \put(5111,3061){\makebox(0,0)[l]{\strut{}$Re = 1000$}}%
      \csname LTb\endcsname%%
      \put(5111,2861){\makebox(0,0)[l]{\strut{} }}%
      \csname LTb\endcsname%%
      \put(5111,2661){\makebox(0,0)[l]{\strut{} }}%
      \csname LTb\endcsname%%
      \put(5111,2461){\makebox(0,0)[l]{\strut{} Present }}%
      \csname LTb\endcsname%%
      \put(5111,2261){\makebox(0,0)[l]{\strut{}$Re = 100$}}%
      \csname LTb\endcsname%%
      \put(5111,2061){\makebox(0,0)[l]{\strut{}$Re = 400$}}%
      \csname LTb\endcsname%%
      \put(5111,1861){\makebox(0,0)[l]{\strut{}$Re = 1000$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{Figs/cavity/u_vs_y_2Dghia.pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figs/cavity/u_vs_y_3Dku.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7500.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1078,704){\makebox(0,0)[r]{\strut{}$-0.5$}}%
      \put(1078,1733){\makebox(0,0)[r]{\strut{}$-0.25$}}%
      \put(1078,2762){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(1078,3790){\makebox(0,0)[r]{\strut{}$0.25$}}%
      \put(1078,4819){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \put(1210,484){\makebox(0,0){\strut{}$-0.6$}}%
      \put(1909,484){\makebox(0,0){\strut{}$-0.4$}}%
      \put(2608,484){\makebox(0,0){\strut{}$-0.2$}}%
      \put(3307,484){\makebox(0,0){\strut{}$0$}}%
      \put(4007,484){\makebox(0,0){\strut{}$0.2$}}%
      \put(4706,484){\makebox(0,0){\strut{}$0.4$}}%
      \put(5405,484){\makebox(0,0){\strut{}$0.6$}}%
      \put(6104,484){\makebox(0,0){\strut{}$0.8$}}%
      \put(6803,484){\makebox(0,0){\strut{}$1$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(198,2761){\rotatebox{-270}{\makebox(0,0){\strut{}$y/L$}}}%
      \put(4006,154){\makebox(0,0){\strut{}$u_x$}}%
      \csname LTb\endcsname%%
      \put(4511,3261){\makebox(0,0)[l]{\strut{} }}%
      \csname LTb\endcsname%%
      \put(4511,3061){\makebox(0,0)[l]{\strut{} }}%
      \csname LTb\endcsname%%
      \put(4511,2861){\makebox(0,0)[l]{\strut{}Ku et al. \cite{ku1987pseudospectral}}}%
      \csname LTb\endcsname%%
      \put(4511,2661){\makebox(0,0)[l]{\strut{}256 $\times$ 256 x 8}}%
      \csname LTb\endcsname%%
      \put(4511,2461){\makebox(0,0)[l]{\strut{}256 $\times$ 256 x 16}}%
      \csname LTb\endcsname%%
      \put(4511,2261){\makebox(0,0)[l]{\strut{}256 $\times$ 256 x 32}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{Figs/cavity/u_vs_y_3Dku.pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figs/cavity/w_vs_z_3D.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1078,704){\makebox(0,0)[r]{\strut{}$-0.06$}}%
      \put(1078,1390){\makebox(0,0)[r]{\strut{}$-0.04$}}%
      \put(1078,2076){\makebox(0,0)[r]{\strut{}$-0.02$}}%
      \put(1078,2762){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(1078,3447){\makebox(0,0)[r]{\strut{}$0.02$}}%
      \put(1078,4133){\makebox(0,0)[r]{\strut{}$0.04$}}%
      \put(1078,4819){\makebox(0,0)[r]{\strut{}$0.06$}}%
      \put(1210,484){\makebox(0,0){\strut{}$-0.5$}}%
      \put(2608,484){\makebox(0,0){\strut{}$-0.25$}}%
      \put(4007,484){\makebox(0,0){\strut{}$0$}}%
      \put(5405,484){\makebox(0,0){\strut{}$0.25$}}%
      \put(6803,484){\makebox(0,0){\strut{}$0.5$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(198,2761){\rotatebox{-270}{\makebox(0,0){\strut{}$w$}}}%
      \put(4006,154){\makebox(0,0){\strut{}$z/\Lambda$}}%
      \csname LTb\endcsname%%
      \put(5471,4656){\makebox(0,0)[l]{\strut{} }}%
      \csname LTb\endcsname%%
      \put(5471,4456){\makebox(0,0)[l]{\strut{} }}%
      \csname LTb\endcsname%%
      \put(5471,4256){\makebox(0,0)[l]{\strut{}$\Lambda = 1$}}%
      \csname LTb\endcsname%%
      \put(5471,4056){\makebox(0,0)[l]{\strut{}$\Lambda = 2$}}%
      \csname LTb\endcsname%%
      \put(5471,3856){\makebox(0,0)[l]{\strut{}$\Lambda = 3$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{Figs/cavity/w_vs_z_3D.pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figs/cavity/x_vs_v_2Dghia.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(946,704){\makebox(0,0)[r]{\strut{}$-0.6$}}%
      \put(946,1390){\makebox(0,0)[r]{\strut{}$-0.4$}}%
      \put(946,2076){\makebox(0,0)[r]{\strut{}$-0.2$}}%
      \put(946,2762){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(946,3447){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \put(946,4133){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \put(946,4819){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \put(1078,484){\makebox(0,0){\strut{}$-0.5$}}%
      \put(2509,484){\makebox(0,0){\strut{}$-0.25$}}%
      \put(3941,484){\makebox(0,0){\strut{}$0$}}%
      \put(5372,484){\makebox(0,0){\strut{}$0.25$}}%
      \put(6803,484){\makebox(0,0){\strut{}$0.5$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(198,2761){\rotatebox{-270}{\makebox(0,0){\strut{}$u_y$}}}%
      \put(3940,154){\makebox(0,0){\strut{}$x/L$}}%
      \csname LTb\endcsname%%
      \put(5111,4656){\makebox(0,0)[l]{\strut{} Ghia et al. \cite{ghia1982high}}}%
      \csname LTb\endcsname%%
      \put(5111,4456){\makebox(0,0)[l]{\strut{}$Re = 100$}}%
      \csname LTb\endcsname%%
      \put(5111,4256){\makebox(0,0)[l]{\strut{}$Re = 400$}}%
      \csname LTb\endcsname%%
      \put(5111,4056){\makebox(0,0)[l]{\strut{}$Re = 1000$}}%
      \csname LTb\endcsname%%
      \put(5111,3856){\makebox(0,0)[l]{\strut{} }}%
      \csname LTb\endcsname%%
      \put(5111,3656){\makebox(0,0)[l]{\strut{} }}%
      \csname LTb\endcsname%%
      \put(5111,3456){\makebox(0,0)[l]{\strut{} Present }}%
      \csname LTb\endcsname%%
      \put(5111,3256){\makebox(0,0)[l]{\strut{}$Re = 100$}}%
      \csname LTb\endcsname%%
      \put(5111,3056){\makebox(0,0)[l]{\strut{}$Re = 400$}}%
      \csname LTb\endcsname%%
      \put(5111,2856){\makebox(0,0)[l]{\strut{}$Re = 1000$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{Figs/cavity/x_vs_v_2Dghia.pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Figs/cavity/x_vs_v_3Dku.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(946,704){\makebox(0,0)[r]{\strut{}$-0.6$}}%
      \put(946,1390){\makebox(0,0)[r]{\strut{}$-0.4$}}%
      \put(946,2076){\makebox(0,0)[r]{\strut{}$-0.2$}}%
      \put(946,2762){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(946,3447){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \put(946,4133){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \put(946,4819){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \put(1078,484){\makebox(0,0){\strut{}$-0.5$}}%
      \put(2509,484){\makebox(0,0){\strut{}$-0.25$}}%
      \put(3941,484){\makebox(0,0){\strut{}$0$}}%
      \put(5372,484){\makebox(0,0){\strut{}$0.25$}}%
      \put(6803,484){\makebox(0,0){\strut{}$0.5$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(198,2761){\rotatebox{-270}{\makebox(0,0){\strut{}$u_y$}}}%
      \put(3940,154){\makebox(0,0){\strut{}$x/L$}}%
      \csname LTb\endcsname%%
      \put(4511,4656){\makebox(0,0)[l]{\strut{} }}%
      \csname LTb\endcsname%%
      \put(4511,4456){\makebox(0,0)[l]{\strut{} }}%
      \csname LTb\endcsname%%
      \put(4511,4256){\makebox(0,0)[l]{\strut{}Ku et al. \cite{ku1987pseudospectral}}}%
      \csname LTb\endcsname%%
      \put(4511,4056){\makebox(0,0)[l]{\strut{}256 $\times$ 256 x 8}}%
      \csname LTb\endcsname%%
      \put(4511,3856){\makebox(0,0)[l]{\strut{}256 $\times$ 256 x 16}}%
      \csname LTb\endcsname%%
      \put(4511,3656){\makebox(0,0)[l]{\strut{}256 $\times$ 256 x 32}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{Figs/cavity/x_vs_v_3Dku.pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> Lists.tex <==

% #### Symbols ####
\newglossaryentry{symb:Pi}{
name=$\pi$, type=symbols,
description=A mathematical constant whose value is the ratio of any circle's circumference to its diameter,
sort=symbolpi
}

\newglossaryentry{symb:Phi}{
name=$\varphi$, type=symbols,
description=An angle,
sort=symbolphi
}

\newglossaryentry{symb:Lambda}{
name=$\lambda$, type=symbols,
description=Lambda indicates usually an eigenvalue in linear algebra,
sort=symbollambda
}

% #### Abbreviations ####
\newacronym{toc}{ToC}{Table of Contents}
\newacronym{los}{LoS}{List of Symbols}
\newacronym{loa}{LoA}{List of Abbreviations}
\newacronym{phd}{PhD}{Doctoral}
\newacronym{MS}{MS}{Masters}
%\newacronym{M$}{MS}{Microsoft}
\newacronym{CD}{CD}{Compact Disc}
\newacronym{kaust}{KAUST}{King Abdullah University of Science and Technology}

%An acronym with a glossary entry
\newacronym{AD}{AD}{Active Directory\protect\glsadd{glos:AD}}



% #### Nomenclature terms ####
\newglossaryentry{glos:AD}{
name=Active Directory,
description={Active Directory is the directory service for Windows based networks, that allows central organization and administration of any network resource. It allows a single-sign-on concept independent from network topologies or network protocols. As a prerequisite you need a Windows Server acting as Domain Controller. This computer stores all necessary data, e.g.~usernames and corresponding passwords}
}

\newglossaryentry{glos:RespF}{name=response file, description={A file 
that allows unattended software installation}}



==> Nomenclature.tex <==
%\chapter*{Nomenclature}
%\ \vfill \centerline{\Huge \bf NOMENCLATURE} \vfill \ 

%\addcontentsline{toc}{chapter}{Nomenclature}
%\cleardoublepage

\chapter*{\centerline{ACRONYMS}}
\addcontentsline{toc}{chapter}{Acronyms}
\begin{center}
\begin{tabular}{ll}\hline
\textbf{Symbol} & \textbf{Meaning}\\\hline
NSE & Navier-Stokes Equations\\
DEC & Discrete Exterior Calculus\\
EC & Exterior Calculus\\
PDE & Partial Differential Equation\\
LES & Large Eddy Simulation\\
DNS & Direct Numerical Simulation\\
FT & Fourier Transform\\
FFT & Fast Fourier Transform\\
LDC & Lid-Driven Cavity\\
TGV & Taylor-Green Vortices\\
\hline
\end{tabular}
\end{center}
%\renewcommand{\baselinestretch}{1.75}



==> Nomenclature2.tex <==
\chapter*{\centerline{LIST OF SYMBOLS}}
\addcontentsline{toc}{chapter}{List of Symbols}
\begin{center}
\begin{tabular}{ll}\hline
\textbf{Symbol} & \textbf{Meaning}\\\hline
$\bf u$ & Velocity vector\\
$p$& Pressure\\ 
$\mu$ & Dynamic viscosity\\
$\flat$ & Flat operator\\
$\ast$ & Hodge star operator\\
$d$ & Exterior derivative operator\\
$\wedge$ & Wedge product operator\\
$N$ & Space dimension\\
$\sigma$ & Domain simplex\\
$K$ & Primal simplicial complex\\
$C^k(K)$ & Space of discrete k-forms defined on primal mesh\\
$D^k(\star K)$ & Space of discrete k-forms defined on dual mesh\\
$u$ & Normal velocity\\
$v$ & Tangential velocity\\
$w$ & Velocity component in the $z{\text -}$direction\\
$U$ & Vector of discrete dual velocity 1-forms\\
$V$ & Vector of primal velocity 1-forms\\
$\widehat{u^{\perp}}$ & Fourier transform of the normal velocity in $\perp$-plane\\
$\widehat{v^{\perp}}$ & Fourier transform of the tangential velocity in $\perp$-plane\\
$\widehat{w}$ & Fourier transform of the Velocity component in the $z{\text -}$direction\\
$P^d$ & Vector of dynamic pressure dual 0-forms\\
$W_v$ & Matrix of the tangential velocity 1-form $v$\\
$\widehat{M_{v}}$ & Wedge product between primal 1-form $\widehat{v^{\perp}}$ and 0-form $\ast d \widehat{u^{\perp}}$ \\
%$\widehat{M_{v1}}$ & Wedge product between primal 1-form $\widehat{v^{\perp}}$ and $\ast^{-1}_1\widehat{u^{\perp}}$.\\
$\widehat{M_u}$ & Wedge product between dual 1-form $\widehat{u^{\perp}}$ and dual 0-form $\widehat{w}$\\

\hline
\end{tabular}
\end{center}
%\renewcommand{\baselinestretch}{1.75}

==> Papers.tex <==

% Appendix for Papers

\refstepcounter{chapter}%
\chapter*{\thechapter \quad Papers Submitted and Under Preparation}

$\bullet$ A Abukhwejah, P Jagad, R Samtaney, P Schmid, {``A Hybrid Discrete Exterior Calculus Discretization and Fourier Transform of the Incompressible Navier-Stokes Equations in 3D"}, \emph{Under preparation}.\\
$\bullet$ P Jagad, B Mantravadi, M Wang, A Abukhwejah, R Samtaney, {``A Discrete Exterior Calculus Based Framework for CFD"}, \emph{Submitted World Congress on Computational Mechanics (WCCM-XV)}, 7. 2022.\\
$\bullet$ P Jagad, A Abukhwejah, M Mohamed, R Samtaney, {``A primitive variable discrete exterior calculus discretization of incompressible Navier–Stokes equations over surface simplicial meshes"}, \emph{Submitted to Physics of Fluids}, 1. 2021. \\

